HyperMAN: Hypergraph-enhanced Meta-learning Adaptive Network for Next POI Recommendation

Next Point-of-Interest (POI) recommendation aims to predict users' next locations by leveraging historical check-in sequences. Although existing methods have shown promising results, they often struggle to capture complex high-order relationships and effectively adapt to diverse user behaviors, particularly when addressing the cold-start issue. To address these challenges, we propose Hypergraph-enhanced Meta-learning Adaptive Network (HyperMAN), a novel framework that integrates heterogeneous hypergraph modeling with a difficulty-aware meta-learning mechanism for next POI recommendation. Specifically, three types of heterogeneous hyperedges are designed to capture high-order relationships: user visit behaviors at specific times (Temporal behavioral hyperedge), spatial correlations among POIs (spatial functional hyperedge), and user long-term preferences (user preference hyperedge). Furthermore, a diversity-aware meta-learning mechanism is introduced to dynamically adjust learning strategies, considering users behavioral diversity. Extensive experiments on real-world datasets demonstrate that HyperMAN achieves superior performance, effectively addressing cold start challenges and significantly enhancing recommendation accuracy.

==> tables/statistics_of_datasets.tex <==
\begin{table}[t]
\centering
\addtolength{\tabcolsep}{4pt}
\caption{\footnotesize Statistics of four datasets from Foursquare.}\label{tab1}
\begin{tabular}{c|c|c|c|c|c}
\toprule
& \#Users & \#POIs & \#Check-ins & \#Categories &Sparsity \\ \midrule
NYC  & 16,387  & 56,252 & 511,431     & 420 & \textbf{99.95\%}      \\
SIN & 8,648   & 33,712 & 355,337     & 398 & \textbf{99.88\%}     \\ 
PHO   & 2,945   & 7,247  & 47,980      & 344 &\textbf{99.78\%}       \\
CAL   & 435    & 3,013  & 13,911      & 293  &\textbf{98.94\%}     \\\bottomrule
\end{tabular}
\vspace{-0.25in}
\end{table}
